Deep clustering: On the link between discriminative models and K-means

In the context of recent deep clustering studies, discriminative models dominate the literature and report the most competitive performances. These models learn a deep discriminative neural network classifier in which the labels are latent. Typically, they use multinomial logistic regression posteriors and parameter regularization, as is very common in supervised learning. It is generally acknowledged that discriminative objective functions (e.g., those based on the mutual information or the KL divergence) are more flexible than generative approaches (e.g., K-means) in the sense that they make fewer assumptions about the data distributions and, typically, yield much better unsupervised deep learning results. On the surface, several recent discriminative models may seem unrelated to K-means. This study shows that these models are, in fact, equivalent to K-means under mild conditions and common posterior models and parameter regularization. We prove that, for the commonly used logistic regression posteriors, maximizing the $L_2$ regularized mutual information via an approximate alternating direction method (ADM) is equivalent to a soft and regularized K-means loss. Our theoretical analysis not only connects directly several recent state-of-the-art discriminative models to K-means, but also leads to a new soft and regularized deep K-means algorithm, which yields competitive performance on several image clustering benchmarks.

==> Soft-Kmeans(1)/commands.tex <==
\newcommand{\tr}[1]{\textrm{#1}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\tnr}[1]{{\textnormal{#1}}}
\newcommand{\mb}[1]{{\mathop{\boldsymbol{#1}}}}
\newcommand{\wmb}[1]{\widetilde{\mb{#1}}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathsf{#1}}
\newcommand{\ds}[1]{\mathds{#1}} 
\newcommand{\ms}[1]{\mathds{#1}}
\newcommand{\mbbmss}[1]{\mathbbmss{#1}}
% overlines and underlines
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\oo}[1]{\ov{\ov{#1}}}
\newcommand{\un}[1]{\underline{#1}}
% boldsymbols
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bB}{{\mathop{\boldsymbol{B}}}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bimath}{\boldsymbol{\imath}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bo}{\boldsymbol{o}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bX}{{\mathop{\boldsymbol{X}}}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bone}{\boldsymbol{1}}
% boldsymbol greek (see http://jblevins.org/log/greek)
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\beeta}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}
% Capital boldsymbol greek (see http://jblevins.org/log/greek)
\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

% referencing 
\newcommand{\seqref}[1]{Eq.~(\ref{#1})}  %% special equation referencing
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\ref{#1}~and~\ref{#2}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\secsref}[2]{Secs.~\ref{#1}~and~\ref{#2}}
%\newcommand{\chapref}[1]{Ch.~\ref{#1}}
\newcommand{\chapref}[1]{Chapter~\ref{#1}}
\newcommand{\chapreff}[1]{Article~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\exref}[1]{Example~\ref{#1}}
\newcommand{\theref}[1]{Theorem~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\tabsref}[2]{Tables~\ref{#1}~and~\ref{#2}}

%sums
\newcommand{\qsum}{\sum_{q=1}^{n}}
\newcommand{\qqsum}{\sum_{q=1}^{n-1}}
\newcommand{\ksum}{\sum_{k=1}^{m}}
\newcommand{\kksum}{\sum_{k=1}^{m-1}}
% equations
\newcommand{\eqlab}[2]{\begin{align} \label{#1} #2 \end{align}}
\newcommand{\eq}[1]{\begin{align*} #1 \end{align*}}

% connectors
%\newcommand{\e}{\mr{e}}
\newcommand{\jj}{\jmath}      % imaginary j
\newcommand{\ee}[1]{\e^{(#1)}}
\newcommand{\ie}{i.e.,~} 		%note the comma and the space (~)
\newcommand{\eg}{e.g.,~}	%note the comma and the space (~)
\newcommand{\cf}{cf.~}		%note the space (~)

%% Editing commands
\newcommand{\ls}[1]{{\color{green} #1}}
\newcommand{\md}[1]{{\color{blue} #1}}
\newcommand{\mustapha}[1]{{\color{blue} #1}}
\newcommand{\mlt}[1]{{\color{red} #1}}
\newcommand{\rs}[1]{{\color{red} #1}}
\newcommand{\tocheck}[1]{\footnote{\color{green} #1}}
\newcommand{\todo}[1]{\footnote{\color{cyan} #1}}

%%%%%% IMPORTANT notation: Mathematical operators
\renewcommand{\emptyset}{\varnothing} % Empty set \varnothing is nicer than \emptyset :)
%\newcommand{\convop}{\mathop{\star}} % LS' preference
\newcommand{\convop}{\mathop{*}} % AA's preference
\newcommand{\argmax}{\mathop{\mr{argmax}}}
\newcommand{\argmin}{\mathop{\mr{argmin}}}
\newcommand{\inv}[1]{{#1}^{-1}}
%\newcommand{\up}[1]{^{(#1)}}  %rapport
\newcommand{\apo}{^{\tnr{apo}}}
\newcommand{\apr}{^{\tnr{a}}}
\newcommand{\ext}{^{\tnr{ext}}}
\newcommand{\mrg}{^{\tnr{mrg}}}
\newcommand{\inn}[2]{\mathop{\langle#1,#2\rangle}\nolimits}
\newcommand{\bdm}{\hat{d}_\mcX}
\newcommand{\ttilde}[1]{\tilde{\tilde{#1}}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\SET}[1]{\left\{#1\right\}}
\newcommand{\bset}[1]{\bigl\{#1\bigr\}}
\newcommand{\cd}{\cdot}
\newcommand{\ld}{\ldots}
\newcommand{\vd}{\vdots}

\newcommand{\e}{\mr{e}}

\newcommand{\hd}[2]{\mathop{d_{\tnr{H}}(#1,#2)}\nolimits}	% Hamming Distance
\newcommand{\hw}[1]{\mathop{w_{\tnr{H}}(#1)}\nolimits}		% Hamming weight

\newcommand{\slopeZCMod}[0]{\mathop{{v}}\nolimits}			% Slope of ZCMod approximation
\newcommand{\interceptZCMod}[0]{\mathop{{q}}\nolimits}		% intercept of ZCMod approximation


\newcommand{\supp}[1]{\mathop{\mathrm{supp}\left(#1\right)}}

\newcommand{\Seq}[1]{\underline{#1}}  %% sequence
\newcommand{\Rv}[1]{#1}   %%% random variable
\newcommand{\SeqRv}[1]{\Seq{\Rv{#1}}}  %% sequence of random var.
\newcommand{\real}[1]{\Re\bigl[#1\bigr]}    % real part
\newcommand{\imag}[1]{\Im\bigl[#1\bigr]}   % imaginary part
\newcommand{\nchoosek}[2]{{{#1} \choose {#2}}}
\newcommand{\sign}[1]{\tr[#1]}   % sign
\newcommand{\mat}[1]{\mathbb{#1}}   
\newcommand{\diag}[1]{\mathop{\mathrm{diag}\left(#1\right)}\nolimits}
\newcommand{\inner}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\PR}[1]{\Pr\SET{#1}}       	% Probability
%\newcommand{\pdf}{\tr{p}}            		% PDF
%\newcommand{\pmf}{\tr{P}}            		% PMF
\newcommand{\pdf}{\mf{p}}            			% PDF. I vote for having the PDFs and the PMFs as italic because the pmf as \tr{P}_\bX(\bX) looks weird and also because I like to see the pmfs and the pdfs as functions, which we denote using italic letters (like the Q-function, f(t), s(t), h(t), etc.)
\newcommand{\bitpmf}{\bp_\tnr{bit}}
\newcommand{\symbolpmf}{\bp}
\newcommand{\bpuni}{\boldsymbol{p}_\tnr{u}}  %%% uniform constellation
\newcommand{\bpbituni}{\boldsymbol{p}_\tnr{bit,u}}  %%% uniform constellation


\newcommand{\pdfCoM}{\tilde{p}{}^\tnr{CoM}}
\newcommand{\pdfZcM}{\tilde{p}{}^\tnr{ZcM}}
\newcommand{\pmf}{P}            			% PMF
\newcommand{\cdf}{F}            			% CDF
\newcommand{\ccdf}{F^\tnr{c}}            			% complementary CDF 

%\newcommand{\Ex}[1]{\ms{E}\set{#1}}    % Expectation.
%\newcommand{\IND}[1]{\ms{I}_{[#1]}}   	% Indicator function
%\newcommand{\IND}[1]{I_{[#1]}}   	% Indicator function
\newcommand{\IND}[1]{\ms{I}\big[{#1}\big]}   	% Indicator function
\newcommand{\Ex}{\ms{E}}     			% Expectation (AA).
\newcommand{\T}{^{\mr{T}}}            		% transpose
\newcommand{\Th}{^{\mr{H}}}             		% Hermitian transpose 
%\newcommand{\dd}{\mr{d}}             		% LS: differentiation operator 
\newcommand{\dd}{\,\mr{d}}             		% LS: differentiation operator (\, added to make it nicer)
\newcommand{\GMI}{^\tnr{GMI}}        	% LS: index
\newcommand{\PSK}{\tnr{PSK}}            % LS: index
\newcommand{\QAM}{\tnr{QAM}}             	% LS: index
\newcommand{\LP}{\mf{P}}             	% Laplace tranform of pdf

% TCM paper
\newcommand{\dE}{d}
\newcommand{\AdE}{A_{d}}
\newcommand{\BdE}{B_{d}}

\newcommand{\MSxteen}{\tnr{M}$16$}

% Alphabets
\newcommand{\MPSK}[1]{$#1$-\tnr{PSK}}	% M-PSK
\newcommand{\MPAM}[1]{$#1$-\tnr{PAM}}	% M-PAM
\newcommand{\MQAM}[1]{$#1$-\tnr{QAM}}	% M-QAM

\newcommand{\BWDS}{{\matB}}             	% bit-wise distance spectrum (UEP chapter)


% Sets often used
% Caligraphics Capital
\newcommand{\mcA}{\mc{A}}
\newcommand{\mcB}{\mc{B}}
\newcommand{\mcC}{\mc{C}}
\newcommand{\mcD}{\mc{D}}
\newcommand{\mcE}{\mc{E}}
\newcommand{\mcF}{\mc{F}}
\newcommand{\mcG}{\mc{G}}
\newcommand{\mcH}{\mc{H}}
\newcommand{\mcI}{\mc{I}}
\newcommand{\mcJ}{\mc{J}}
\newcommand{\mcK}{\mc{K}}
\newcommand{\mcL}{\mc{L}}
\newcommand{\mcM}{\mc{M}}
\newcommand{\mcN}{\mc{N}}
\newcommand{\mcO}{\mc{O}}
\newcommand{\mcP}{\mc{P}}
\newcommand{\mcQ}{\mc{Q}}
\newcommand{\mcR}{\mc{R}}
\newcommand{\mcS}{\mc{S}}
\newcommand{\mcT}{\mc{T}}
\newcommand{\mcU}{\mc{U}}
\newcommand{\mcV}{\mc{V}}
\newcommand{\mcW}{\mc{W}}
\newcommand{\mcX}{\mc{X}}
\newcommand{\mcY}{\mc{Y}}
\newcommand{\mcZ}{\mc{Z}}
\newcommand{\mcCr}{\mc{K}}
% Caligraphics Small
\newcommand{\mca}{\mc{a}}
\newcommand{\mcb}{\mc{b}}
\newcommand{\mcc}{\mc{c}}
\newcommand{\mcd}{\mc{d}}
\newcommand{\mce}{\mc{e}}
\newcommand{\mcf}{\mc{f}}
\newcommand{\mcg}{\mc{g}}
\newcommand{\mch}{\mc{h}}
\newcommand{\mci}{\mc{i}}
\newcommand{\mcj}{\mc{j}}
\newcommand{\mck}{\mc{k}}
\newcommand{\mcl}{\mc{l}}
\newcommand{\mcm}{\mc{m}}
\newcommand{\mcn}{\mc{n}}
\newcommand{\mco}{\mc{o}}
\newcommand{\mcp}{\mc{p}}
\newcommand{\mcq}{\mc{q}}
\newcommand{\mcr}{\mc{r}}
\newcommand{\mcs}{\mc{s}}
\newcommand{\mct}{\mc{t}}
\newcommand{\mcu}{\mc{u}}
\newcommand{\mcv}{\mc{v}}
\newcommand{\mcw}{\mc{w}}
\newcommand{\mcx}{\mc{x}}
\newcommand{\mcy}{\mc{y}}
\newcommand{\mcz}{\mc{z}}

\newcommand{\msA}{\ms{A}}
\newcommand{\msL}{\ms{L}}

\newcommand{\mfa}{\mf{a}}
\newcommand{\mfb}{\mf{b}}
\newcommand{\mfc}{\mf{c}}
\newcommand{\mfd}{\mf{d}}
\newcommand{\mfe}{\mf{e}}
\newcommand{\mff}{\mf{f}}
\newcommand{\mfg}{\mf{g}}
\newcommand{\mfh}{\mf{h}}
\newcommand{\mfi}{\mf{i}}
\newcommand{\mfj}{\mf{j}}
\newcommand{\mfk}{\mf{k}}
\newcommand{\mfl}{\mf{l}}
\newcommand{\mfm}{\mf{m}}
\newcommand{\mft}{\mf{t}}
\newcommand{\mfs}{\mf{s}}
\newcommand{\mfw}{\mf{w}}
\newcommand{\mfx}{\mf{x}}
\newcommand{\mfy}{\mf{y}}
\newcommand{\mfz}{\mf{z}}

\newcommand{\mfD}{\mf{D}}
\newcommand{\mfI}{\mf{I}}
\newcommand{\mfJ}{\mf{J}}
\newcommand{\mfM}{\mf{M}}
\newcommand{\mfR}{\mf{R}}
\newcommand{\mfK}{\mf{K}}
\newcommand{\mfX}{\mf{X}}

\newcommand{\Real}{\mathbb{R}}		% R (The real,natural, etc. should used blackboard bold fonts... \mathbb{})
\newcommand{\Complex}{\mathbb{C}}		% R (The real,natural, etc. should used blackboard bold fonts... \mathbb{})
\newcommand{\Natural}{\mathbb{N}}		% N
\newcommand{\RealN}{\mathbb{R}^N}	% R^N
\newcommand{\Zplus}{\mathbb{Z}^+}	% Z^+
\newcommand{\Binary}{\mathbb{B}}	% Binary Set
% Alphabets
\newcommand{\mcXPSK}[1]{\mcX_{#1\tnr{-PSK}}}
\newcommand{\mcXPAM}[1]{\mcX_{#1\tnr{-PAM}}}
\newcommand{\mcXQAM}[1]{\mcX_{#1\tnr{-QAM}}}
% Ordered Alphabets
\newcommand{\matXPSK}[1]{\matX_{#1\tnr{-PSK}}}
\newcommand{\matXPAM}[1]{\matX_{#1\tnr{-PAM}}}
\newcommand{\matXQAM}[1]{\matX_{#1\tnr{-QAM}}}

% Matrices often used
\newcommand{\II}[1]{\tnr{\textbf{I}}_{[#1]}}   		% Identity matrix....
% Matrices %old. New notation below
%\newcommand{\matA}{\mat{A}}
%\newcommand{\matB}{\mat{B}}
%\newcommand{\matC}{\mat{C}}
%\newcommand{\matD}{\mat{D}}
%\newcommand{\matE}{\mat{E}}
%\newcommand{\matF}{\mat{F}}
%\newcommand{\matG}{\mat{G}}
%\newcommand{\matH}{\mat{H}}
%\newcommand{\matI}{\mat{I}}
%\newcommand{\matJ}{\mat{J}}
%\newcommand{\matK}{\mat{K}}
%\newcommand{\matL}{\mat{L}}
%\newcommand{\matM}{\mat{M}}
%\newcommand{\matN}{\mat{N}}
%\newcommand{\matO}{\mat{O}}
%\newcommand{\matP}{\mat{P}}
%\newcommand{\matQ}{\mat{Q}}
%\newcommand{\matR}{\mat{R}}
%\newcommand{\matS}{\mat{S}}
%\newcommand{\matT}{\mat{T}}
%\newcommand{\matU}{\mat{U}}
%\newcommand{\matV}{\mat{V}}
%\newcommand{\matW}{\mat{W}}
%\newcommand{\matX}{\mat{X}}
%\newcommand{\matY}{\mat{Y}}
%\newcommand{\matZ}{\mat{Z}}
%% New notation
%\newcommand{\matA}{\ba}
%\newcommand{\matB}{\bb}
%\newcommand{\matC}{\bc}
%\newcommand{\matD}{\bd}
%\newcommand{\matE}{\be}
%\newcommand{\matF}{\bf}
%\newcommand{\matG}{\bg}
%\newcommand{\matH}{\bh}
%\newcommand{\matI}{\bi}
%\newcommand{\matJ}{\bj}
%\newcommand{\matK}{\bk}
%\newcommand{\matL}{\bl}
%\newcommand{\matM}{\bm}
%\newcommand{\matN}{\bn}
%\newcommand{\matO}{\bo}
%\newcommand{\matP}{\bp}
%\newcommand{\matQ}{\bq}
%\newcommand{\matR}{\br}
%\newcommand{\matS}{\bs}
%\newcommand{\matT}{\bt}
%\newcommand{\matU}{\bu}
%\newcommand{\matV}{\bv}
%\newcommand{\matW}{\bw}
%\newcommand{\matX}{\bx}
%\newcommand{\matY}{\by}
%\newcommand{\matZ}{\bz}

% New^2 notation
\newcommand{\matA}{\tnr{\textbf{A}}}
\newcommand{\matB}{\tnr{\textbf{B}}}
\newcommand{\matC}{\tnr{\textbf{C}}}
\newcommand{\matD}{\tnr{\textbf{D}}}
\newcommand{\matE}{\tnr{\textbf{E}}}
\newcommand{\matF}{\tnr{\textbf{F}}}
\newcommand{\matG}{\tnr{\textbf{G}}}
\newcommand{\matH}{\tnr{\textbf{H}}}
\newcommand{\matI}{\tnr{\textbf{I}}}
\newcommand{\matJ}{\tnr{\textbf{J}}}
\newcommand{\matK}{\tnr{\textbf{K}}}
\newcommand{\matL}{\tnr{\textbf{L}}}
\newcommand{\matM}{\tnr{\textbf{M}}}
\newcommand{\matN}{\tnr{\textbf{N}}}
\newcommand{\matO}{\tnr{\textbf{O}}}
\newcommand{\matP}{\tnr{\textbf{P}}}
\newcommand{\matQ}{\tnr{\textbf{Q}}}
\newcommand{\matR}{\tnr{\textbf{R}}}
\newcommand{\matS}{\tnr{\textbf{S}}}
\newcommand{\matT}{\tnr{\textbf{T}}}
\newcommand{\matU}{\tnr{\textbf{U}}}
\newcommand{\matV}{\tnr{\textbf{V}}}
\newcommand{\matW}{\tnr{\textbf{W}}}
\newcommand{\matX}{\tnr{\textbf{X}}}
\newcommand{\matY}{\tnr{\textbf{Y}}}
\newcommand{\matZ}{\tnr{\textbf{Z}}}

%%%%%% IMPORTANT notation: VARIABLES 

\newcommand{\lk}{l_{k}}  % kth L-value
\newcommand{\Lk}{L_{k}}  % kth L-value (r.v.)
\newcommand{\Bk}{B_{k}}  % kth bit (r.v.)
\newcommand{\lktilde}{\tilde{l}_{k}}  % kth L-value
\newcommand{\lkapo}{l_{k}\apo}  % kth a posteriori L-value
\newcommand{\lkapr}{l_{k}\apr}  % kth a priori L-value
\newcommand{\lkpapr}{l_{k'}\apr}  % k'th a priori L-value

\newcommand{\CSI}{\mathsf{csi}}  %%% SNR
\newcommand{\CSIrv}{\mathsf{CSI}}  %%% SNR random variable
\newcommand{\corSNR}{\delta}  % Doppler frequency
\newcommand{\fD}{f_\text{D}}  % Doppler frequency

\newcommand{\SNR}{\mathsf{snr}}  %%% SNR
\newcommand{\SNRrv}{\mathsf{SNR}}  %%% SNR random variable
\newcommand{\SNRav}{\ov{\mathsf{snr}}}  %%% SNR
\newcommand{\SNRvec}{\boldsymbol{\mathsf{snr}}}  %%% SNR
\newcommand{\SNRrvvec}{\boldsymbol{\mathsf{SNR}}}  %%% SNR
\newcommand{\Pav}{\ov{P}}  %%% Average power
\newcommand{\gMI}{\mathsf{GMI}}  %%% SNR


\newcommand{\mNak}{\mf{m}}%{m_\tnr{f}}}  %%% parameter of the Nakagami-m fading
\newcommand{\SIR}{\mathsf{sir}}  %%% SIR
\newcommand{\SINR}{\mathsf{sinr}}  %%% SINR
\newcommand{\SINRrv}{{\mathsf{SINR}}}  %%% SINR random variable
\newcommand{\SIRav}{\ov{\mathsf{sir}}}  %%% SIR average
\newcommand{\PEP}{\mr{PEP}}  %%% PEP
\newcommand{\UB}{\tnr{UB}}  %%% Upper Bound
\newcommand{\BER}{\mr{BER}}  %%% BER
\newcommand{\PER}{\mr{PER}}  % packet error rate
\newcommand{\HBER}{\mr{ber}_{\tnr{hard}}}   %%% BER based on hard decision
\newcommand{\bdij}{\bd}  %%% distance between the constellation symbols
\newcommand{\dl}{\delta_l}  %%% l-th ED in the constellation
\newcommand{\ED}{\delta}  %%% ED
\newcommand{\Lij}{\mf{L}}  %%% linear form, line in the observation space
\newcommand{\Eb}{E_\tnr{b}}  	% Energy per bit
\newcommand{\EB}{\mathsf{EB}}
\newcommand{\Es}{E_\tnr{s}}  	% Energy per symbol
\newcommand{\X}{\mcX}	% constellation
\newcommand{\mcXku}{\X_{k,u}}	% Subconstellations
\newcommand{\mcXkb}{\X_{k,b}}	% Subconstellations
\newcommand{\mcXkz}{\X_{k,0}}	% Subconstellations k,Zero
\newcommand{\mcXko}{\X_{k,1}}	% Subconstellations k,One

\newcommand{\mcIXku}{\mc{I}_{k,u}}	% Indices Subconstellations
\newcommand{\mcIXkb}{\mc{I}_{k,b}}	% Indices Subconstellations
\newcommand{\mcIXkz}{\mc{I}_{k,0}}	% Indices Subconstellations k,Zero
\newcommand{\mcIXko}{\mc{I}_{k,1}}	% Indices Subconstellations k,One


\newcommand{\mcXsub}[2]{\X_{#1,#2}}	% Subconstellations with parameters
\newcommand{\x}{\bx} 	% constellation symbol
\newcommand{\B}{\mcB}     		% set of labels
\newcommand{\C}{\mcC_\bB}     			% Codebook (bits)
\newcommand{\Cx}{\mcC_{\bX}}     		% Codebook (symbols)
\newcommand{\Cxk}[1]{\mcC_{\bX,#1}}     		% Codebook (symbols)
\newcommand{\Cc}{\mcC_{\bC}}     		% Codebook (coded bits)
%\newcommand{\benc}{\mbbmss{C}} 		% Binary Encoder
%\newcommand{\benc}{\mbbmss{B}} 		% Binary Encoder
\newcommand{\benc}{\matG} 		% Binary Encoder
%\newcommand{\benc}{\matB} 		% Binary Encoder
%\newcommand{\labeling}{\mbbmss{L}} 		% Binary Labeling
%\newcommand{\labeling}{\matL} 		% Binary Labeling
\newcommand{\labeling}{\matQ} 		% Binary Labeling
\newcommand{\R}{R}           	% spectral efficiency element
\newcommand{\W}{\mf{W}}              	% Bandwidth of the signals
\newcommand{\No}{\mf{N}_{0}}             % power of the noise for rapport
%\newcommand{\EE}{\mf{E}_\tr{eff}}    % Energy effciency
%\newcommand{\EEmin}{\mf{E}_\tr{eff,min}}    % minimum Energy effciency
\newcommand{\Rt}{\mf{R}}              % transmission rate : \Nb/(Ns\Ts)
\newcommand{\Rc}{R_\tnr{c}}  	% binary code rate =\kc/nc
\newcommand{\SCR}{\mf{S}}  	% scrambler
\newcommand{\kc}{k_\tnr{c}}  	% 
\newcommand{\nc}{n_\tnr{c}}  	% 
\newcommand{\Nbl}[1]{{ \mathop{ N_{\tnr{b},#1} } }} 	% number of bits in the block
\newcommand{\Nb}{{\mathop{N_\tnr{b}}}} 	% number of bits in the packet
\newcommand{\Ns}{{\mathop{N_\tnr{s}}}} 	% number of symbols in the block
\newcommand{\Ncrc}{{\mathop{N_\tnr{crc}}}} 	% number of CRC bits 
\newcommand{\Nsf}{{\mathop{N_{\tnr{s},1}}}} 	% number of symbols in the first block

\newcommand{\Ts}{T_\tnr{s}} 	% Symbol period
%\newcommand{\Rs}{R_\tnr{s}} 	% Symbol rate
\newcommand{\bit}{\tnr{bit}} 	% bit (unit)
\newcommand{\second}{\tnr{s}} % s (unit)
\newcommand{\symb}{\tnr{symbol}} % s (unit)
\newcommand{\Nc}{N_\tnr{c}} 	% number of coded bits
\newcommand{\m}{m}             	% number of bits in the label
\newcommand{\M}{M}             	% M=2^{\m} = |\X|  number of symbols in the constellation
\newcommand{\K}{K}              	% \K=dim(\X) number of dimensions in the constellation, K=2 complex, K=1 real 
\newcommand{\Kp}{K'}              % \K=dim(\X) number of dimensions of the received signal  
\newcommand{\Zj}{\mcY}      % decision region
\newcommand{\WW}{\mcW}      % wedge
\newcommand{\Nt}{N_\tnr{t}}      % MIMO notation : # of transmitted symbols
\newcommand{\Nr}{N_\tnr{r}}      % MIMO notation : # of received symbols
\newcommand{\hf}{\mf{H}}      % function : the integral over the wedge or the half-space

\newcommand{\nthmetric}{\mbbmss{m}} 	% nth metric
\newcommand{\Nthmetric}{\mbbmss{M}} 	% nth metric (r.v.)
\newcommand{\totmetric}{\mbbmss{M}} 	% total (accumulated) metric

%%% HARQ notation
\newcommand{\RR}{\tr{rr}} 	
\newcommand{\IR}{\tnr{ir}}
\newcommand{\SC}{\tnr{SC}}  %%% superposition coding
\newcommand{\TS}{\tnr{TS}}  %%% time sharing
\newcommand{\VL}{\tnr{VL}}  %%%variable length
\newcommand{\VP}{\tnr{VP}}  %%%variable power
\newcommand{\IRHARQ}{\tr{IR-HARQ}}  	
\newcommand{\I}{\tr{I}} 	
\newcommand{\PHY}{\tr{PHY}}
\newcommand{\AMC}{\tr{AMC}}
\newcommand{\amc}{\tnr{amc}}
\newcommand{\HARQ}{\tr{HARQ}}
\newcommand{\Err}{\mf{ERR}}
\newcommand{\Errb}[1]{\mf{ERR}^{\tnr{b}}_{#1}}       % parity rate
\newcommand{\ack}{\mf{ACK}}  %%% message ACK
\newcommand{\nack}{\mf{NACK}}  %% message NACK
\newcommand{\kmax}{K}		%% maximum number of transmissionsfg
\newcommand{\kk}{k}
\newcommand{\sk}{[k]}   %%% 
\newcommand{\cu}{\tr{cu}}  %% per channel use
\newcommand{\ti}{\tr{ti}}  %% per time interval
\newcommand{\ovh}{\tr{ovh}}  %% overhead
\newcommand{\tot}{\tr{tot}}  %% total
\newcommand{\sbrq}{\tr{sbrq}} %systematic backtrack
\newcommand{\ansbrq}{\tr{ansbrq}} %All-or-None systematic backtrack
\newcommand{\Lc}{\tr{L}} %layer coding
\newcommand{\AN}{\tr{AoN}} %layer coding
\newcommand{\xp}{\tnr{xp}}
\newcommand{\hol}{\ell}		%% HoL index
\newcommand{\Tarq}{\mcD }  %%% packet transmission time  at ARQ level
\newcommand{\Tharq}{\mcT }  %%% packet transmission time  at HARQ level
\newcommand{\kkrv}{\mcK }  %%% number of packet transmissions at HARQ level
\newcommand{\EE}{\mathsf{EE}}
\newcommand{\SEE}{\mathsf{S}}
\newcommand{\EEmin}{\EE_{\min}}
\newcommand{\EEdB}{\EE_{\tnr{dB}}}
\newcommand{\EBdB}{\EB^{\tnr{dB}}}
\newcommand{\EBmindB}{\EB_{\tnr{min}}^{\tr{dB}}}
\newcommand{\EBmin}{\EB_{\tnr{min}}}
\newcommand{\Iv}{\mathbf{I}}
\newcommand{\Mv}{\mathbf{M}}
\newcommand{\kv}{\mathbf{k}}	
\newcommand{\tsm}{\tnr{TSM}}
\newcommand{\scm}{\tnr{SCM}}	
\newcommand{\holxt}{\ell'}

\newcommand{\sumk}{\sum_{k=1}^{\K}}  %% sum_k->(K)
\newcommand{\sumki}{\sum_{k=1}^{\infty}}  %% sum_k->inf
\newcommand{\fK}{f_\K}  %% f_K
\newcommand{\Isig}{I^\Sigma}  %% I^\Sigma (cumulated MI)
\newcommand{\Rsig}{\R^\Sigma}  %% R^\Sigma (cumulated rate)

\newcommand{\Ro}{Re}  
\newcommand{\Eharqa}{\mc{E}_{\ack}}
\newcommand{\Eharq}{\mc{E}}
\newcommand{\Eharqn}{\mc{E}_{\nack}}
\newcommand{\TmI}{T_{I} } 
\newcommand{\TmR}{T_{R} } 
\newcommand{\TmP}{T_{P} }  %%% # of discretization points of $P$

\newcommand{\Nsk}[1]{\mathop{N_{\tnr{s},#1}}} 	% number of symbols in the block
%\newcommand{\Rs}[1]{\mathop{\rho_{\tnr{s},#1}}}       % parity rate
\newcommand{\Rs}[1]{\mathop{\rho_{#1}}}       % parity rate

\newcommand{\aoneP}{\mf{1P}}  %%% encoding action 1P
\newcommand{\azeroP}{\mf{0P}}  %%% encoding action 0P
\newcommand{\aTS}{\mf{TS}}  %%% encoding action TS
\newcommand{\aSC}{\mf{SC}}  %%% encoding action SC
\newcommand{\mAN}{\mf{M}}  %%% variable for the binary message ACK/NACK

%%
\newcommand{\WEP}{\mf{WEP}}  % word-error probability (coded)
\newcommand{\DECwo}{\mr{DEC}}  % decoding function
\newcommand{\DECbwo}{\mr{DEC}^\tnr{b}}  % binary decoding function
\newcommand{\DEC}[1]{\DECwo[#1]}  % decoding function
\newcommand{\DECb}[1]{\DECbwo[#1]}  % binary decoding function

\newcommand{\ENCwo}{\mr{ENC}}  % encoding function
\newcommand{\ENCbwo}{\mr{ENC}^\tnr{b}}  % binary encoding function
\newcommand{\ENC}[1]{\ENCwo [#1]}  % encoding function
\newcommand{\ENCb}[1]{\ENCbwo [#1]}  % binary encoding function

\newcommand{\MOD}[1]{\Phi[#1]}      % modulator operation 
\newcommand{\MODwo}{\Phi}      		% modulator operation without arguments
\newcommand{\MODwoa}{\Phi}  
\newcommand{\DEM}[2]{L(#2,#1)}      		% demodulator (L-values calculation) operation 
 \newcommand{\MODMP}{\Phi^{\tnr{MP}}}  
\newcommand{\DEMs}[2]{L^\Sigma(#2,#1)}      		% demodulator (L-values calculation) operation 
\newcommand{\DEMwo}{\Theta}      		% demodulator (L-values calculation) operation 
\newcommand{\HDET}[1]{\hat{\Phi}^{-1}\set{#1}}      % modulator operation 

\newcommand{\qmetric}{\mathbb{q}}
\newcommand{\qq}{\qmetric} 		% mismatched decoding metric

\newcommand{\dBval}{\tnr{dB}} % dB (numerical value)
\newcommand{\dB}{~\tnr{[dB]}} % dB (value)
\newcommand{\bpcu}{\tnr{[bit/cu]}} % bit per channel use (unit)
\newcommand{\bpcuval}{\tnr{bit/cu}} % bit per channel use (unit)


%\newcommand{\blue}[1]{{\color{blue}#1}}
%\newcommand{\red}[1]{{\color{red}#1}}
%\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\magenta}[1]{{\color{magenta}#1}}

\newenvironment{blockwhite}[0]
{\begin{beamerboxesrounded}[upper=black,lower=red,shadow=true]}
{\end{beamerboxesrounded}}

==> Soft-Kmeans(1)/included_packages.tex <==
\usepackage{amsmath,amssymb,amscd,latexsym,dsfont,wasysym,bbm}
\usepackage{txfonts}  %% transforms the fonts into Times-New-Roman style
\usepackage{float}
\usepackage{color}
\usepackage{graphicx,subfigure}
\usepackage{multirow,multicol} 
\usepackage{verbatim}
\usepackage{psfrag}
\usepackage{comment}
\usepackage{makeidx}
\usepackage[]{algorithm}
\usepackage{algorithmic}
\usepackage{cite}
\usepackage{cases}
\usepackage{amsthm}
 \usepackage{setspace}
%\usepackage[table]{xcolor}
\usepackage{pgfplots} %%%% added by LS for the errata 7.sept.2015
%\usepackage{subdepth}				% To fix the alignment of the subscripts. It helps, but it also makes {?BICM-ID.SumExp.m1} look horrible!

==> included_packages.tex <==
\usepackage{amsmath,amssymb,amscd,latexsym,dsfont,wasysym,bbm}
\usepackage{txfonts}  %% transforms the fonts into Times-New-Roman style
\usepackage{float}
\usepackage{color}
\usepackage{graphicx,subfigure}
\usepackage{multirow,multicol} 
\usepackage{verbatim}
\usepackage{psfrag}
\usepackage{comment}
\usepackage{makeidx}
\usepackage[]{algorithm}
\usepackage{algorithmic}
\usepackage{cite}
\usepackage{cases}
\usepackage{amsthm}
 \usepackage{setspace}
%\usepackage[table]{xcolor}
\usepackage{pgfplots} %%%% added by LS for the errata 7.sept.2015
%\usepackage{subdepth}				% To fix the alignment of the subscripts. It helps, but it also makes {?BICM-ID.SumExp.m1} look horrible!
